GPUs, CPUs, and... NICs: Rethinking the Network's Role in Serving Complex AI Pipelines

The increasing prominence of AI necessitates the deployment of inference platforms for efficient and effective management of AI pipelines and compute resources. As these pipelines grow in complexity, the demand for distributed serving rises and introduces much-dreaded network delays. In this paper, we investigate how the network can instead be a boon to the excessively high resource overheads of AI pipelines. To alleviate these overheads, we discuss how resource-intensive data processing tasks -- a key facet of growing AI pipeline complexity -- are well-matched for the computational characteristics of packet processing pipelines and how they can be offloaded onto SmartNICs. We explore the challenges and opportunities of offloading, and propose a research agenda for integrating network hardware into AI pipelines, unlocking new opportunities for optimization.

==> conclusion.tex <==
\section{conclusion}


CPU overheads for vision pipeline data processing tasks are prohibitively high thereby hurting SLOs.
We explore offloading these data processing onto programmable network hardware, which can reap significant performance wins.
We hope this work prompts further investigation in leveraging programmable network hardware for alleviating worsening bottlenecks.

==> design.tex <==

\section{Design}
\label{s:offloading}

\subsection{NetFPGA background}

In this paper, we use the NetFPGA-SUME SmartNIC based on the XC7VX690T FPGA with 10G Ethernet ports.
We believe that our system design is not unique to this architecture and can be applied to other SmartNIC models, and we plan to explore ASIC~\cite{pensando}, SoC~\cite{bluefield}, and other FPGA~\cite{xilinx-alveo} SmartNIC models in future work.

Within the NetFPGA, packets are moved through a pipeline of packet-processing modules using the AXI4-Stream protocol.
%NetFPGA's AXI4-Stream protocol uses a data bus width of 32 bytes.
%Thus a packet is broken up into multiple 32-byte AXI4-Stream transmissions, with a module processing one transmission per clock cycle.
NetFPGA's AXI4-Stream protocol uses a data bus width of 32 bytes that can be processed in a single clock cycle.
%\uab{Cutting since we already state the frequency}
%The clock cycle of the base NetFPGA design is 5 ns, although this naturally increases with the complexity of the design.
%The end of a packet is signaled by a specific flag that travels on a parallel wire between modules.
The NetFPGA project provides modules to read and write packets from Ethernet ports; custom logic can be inserted between these modules.


\subsection{Design overview}

We designed an example pre-processor to offload the high CPU utilization tasks seen in \S\ref{sec:motivation}.
End-to-end, this pre-processor takes as input a video stream of the environment captured by the device camera.
It outputs a sequence of tensors that can be input into one of the backend vision pipelines.
This pre-processor consists of 6 components arranged in an FPGA pipeline: video decoding, RGB image conversion, cropping, resizing, image-to-tensor conversion, and normalization.

The first stage is a video decoder. Hardware accelerators for video decoding are common in practice, and several companies organizations offer pre-built video decoder IP cores for common formats, like H.264~\cite{h264-overview, h264-decoder-ip}. After the video is decoded into video frames, the following stage converts frames from the decoded video stream into RGB images. Each RGB image is then resized by discarding pixels that fall outside of a given boundary and image metadata is updated accordingly. The resize stage then changes the height and width of each image using bilinear interpolation. The next stage involves the \texttt{ToTensor} operation, which converts an RGB image to a tensor which is composed of two parts. First, the RGB bitmap array ($\textit{Height} \times \textit{Width} \times \textit{Color}$) is converted to have shape $\textit{Color} \times \textit{Height} \times \textit{Width}$ array. Second, pixel intensity values are scaled from [0, 255] to [0.0, 1.0] by dividing each pixel value by 255. Lastly, the normalize stage which implements the \texttt{Normalize} function executes on all individual color channels by subtracting the mean from a pixel's intensity value and divides the result by the standard deviation to get normalized intensities. The means and standard deviations are typically provided a priori and are not computed on the FPGA.

\subsection{Implementation}
Our vision pipelines cannot ingest raw RGB bitmap images so our image-to-tensor converter converts these RGB bitmap arrays into tensor values for inference. 
Aligning with the \texttt{ToTensor} implementation, the converter reshapes arrays from an input $\textit{Height} \times \textit{Width} \times \textit{Color}$ array to an output $\textit{Color} \times \textit{Height} \times \textit{Width}$ array. To reshape arrays, we first need to extract the red, green, and blue channels separately before converting the pixel intensities in each channel to 32-bit floating point values.  Then the tensor floats for one channel are output one at a time. 

To perform this extraction, the \texttt{reshaper} module feeds the AXI stream into three \texttt{channel\_extractor} modules, each of which extracts the intensity values (represented as unsigned 8-bit integers) for a single predefined color channel (red, green, or blue), by only keeping every third byte, dropping all remaining bytes. These streams are each buffered in a FIFO queue, all of which are accessed by a single \texttt{arbiter} module. The \texttt{arbiter} forwards the red, blue, and green streams to the \texttt{scaler} in that order. The \texttt{reshaper} module transmits pixel intensities to the \texttt{scaler} module one channel/color at a time. I.e., in an RGB image, the red channel must first be processed before the green and blue channels. The green and blue channels are first buffered and cannot begin being transmitted until the red channel has been finished processing. Thus, the channel buffers must be large enough to store the pixel values of at least a full image.


Afterwards, each 8-bit integer needs to be converted into a 32-bit float that falls within the range [0.0, 1.0].
We precompute a 256-entry lookup table to map each 8-bit positive integer $i$ into the respective 32-bit IEEE 754 FP representation of $i/256$. 
The translation from 8-bit integers to 32-bit floats expands the data size of the output from 8 bits to 32 bits.
This expansion necessitates the processing of frames at an ingress throughput substantially lower than the capacity of the incoming Ethernet link, leaving it underutilized. 








==> discussion.tex <==
% Future compiler problems in this space: compiling offloads to NIC implementations automatically.
One interesting area for future work is automatically compiling an idealized specification of offload functionality to a SmartNIC implementation of that functionality. Concretely, the specification could be a function written in an imperative programming language that takes as input an application data unit (ADU)~\cite{clark_tenenhouse} that represents a chunk of data that can be processed by an application independently of other chunks. Depending on the context, example ADUs could be prompts (or sentences within a prompt), entire images, a feature vector, a single frame of video, or a single (or multiple) sensor readings. The specification could be written with no restrictions on the size of an individual ADU, the amount of memory the ADU accesses to carry out the specification, or what kinds of computations are permitted within the specification. By contrast, \emph{the implementation} has to contend with size limits on packets (e.g., an MTU), computational constraints (e.g., to permit line rate operation), and memory constraints (e.g., limited BRAM on an FPGA). Automatically bridging this semantic gap---in essence, automating what we have manually sketched out in \S\ref{s:offloading} would allow us to automatically offload many data-processing operations.

\section{Discussion}
\label{s:discussion}
\as{I agree with Mike. The data source was more relevant in the context of the previous edge AI based framing. This one doesn't exactly have the concept of a data source.}
\Para{Offloading to the data source.} \mw{Is this necessary? For this submission, I think the benefits of offloading to the NIC over the data source are much more apparent} One alternative offload candidate is the data source itself (e.g., mobile device or surveillance camera) because of its close proximity to the data, but its localized poor vantage point makes it suboptimal for inference servers. 
Devices cannot make global optimization decisions across multiple video feeds and do not have access to private resource utilization data on the server to guide the aggressiveness of optimizations.
Further, data processing operations often expand the size of the data sample. For example, image processing operations require the data to be represented as larger floating points rather than integers while text processing uses numerical tokens which are larger than the original text, resulting in high bandwidth consumption from the device to the server.
Lastly, the close proximity to the compute server enables the on-path programmable network hardware to be used for intermediate processing, whereas the data source would be constrained to performing operations either at pipeline start or end.


% In contrast, smart network hardware such as SmartNICs and programmable switches have a global view of all incoming data streams at that edge while also having access to crucial information from the inference server such as queue sizes and latencies, allowing it to make much more intelligible optimization decisions. 
% For example, when the edge server is inundated with requests, a video feed that has less activity over time can be filtered at a higher frequency than other more dynamic video feeds\as{A bit confused. shouldn't we filter the more dynamic video because it is likely to have more interesting stuff?}, while incurring a minimal drop in accuracy.
% Moreover, because the data is not expanded to floats until it reaches the network device, there are no additional network overheads.
% Lastly, the close proximity to the compute server enables the on-path programmable network hardware to be used for intermediate processing, whereas the data source would be constrained to performing operations either at pipeline start or end.

\as{Is the paragraph below connected to the paragraph above?}
We emphasize that data processing operations are highly amenable to network hardware offload.
These operations are normally performed sequentially, and thus can be pipelined. 
For example, the vision tasks involve the \texttt{Resize}, \texttt{Cropping}, \texttt{ToTensor}, and \texttt{Normalize} operations one after the other. Computations within a single operation can be further pipelined, e.g., \texttt{ToTensor} reshapes the image before scaling the pixel values. 
Each computational step is highly amenable to data parallelism since they operate on image representations, which can divided into segments and processed independently.


\Para{Using other in-network accelerators.} In this paper, we have focused primarily on SmartNICs. 
Our designs were targeting an FPGA-based SmartNIC such as the NetFPGA-SUME, but our approach is applicable to other FPGA-based SmartNICs and even other SmartNIC architectures more broadly because of their close proximity to the server and highly parallel processing.
In recent years, programmable network switches (e.g., Tofino \cite{tofino}) have received significant attention.
Although these devices offer a generous degree of programmability to operators while maintaining line-rate packet processing, they currently only process packet headers instead of payloads.
However, they can still be used for other tasks, such as scheduling, and data samples can be embedded in the packet headers for processing, similar to prior switch offload approaches \cite{!!!}.

\as{Yeah, we should ditch switches for this paper. Some of the text below can be removed.}
\Para{Why use network accelerators instead of deploying
more CPU servers? } Because switch \rn{we're punting on switches, right?} and NIC programmability will essentially come for free in the future. Switches and NICs \emph{need} to exist within the edge infrastructure for basic connectivity from the base station to the GPUs via the servers. Both switches and NICs have become increasingly programmable over the years with many commercial products with varying degrees of programmability~\cite{tofino, trident4, bluefield, netfpga, pensando, netronome-agilio}. In the future, we believe programmability in switches and NICs will increasingly be a commodity technology. If programmability is the norm, costs would be minimal---possibly with the exception of managing heterogeneity, which creates an interesting set of research challenges. At the same time, programmable networks can substantially improve application performance---as many prior projects have shown. Simultaneously, offloading functionality into the network frees up existing edge CPUs and improves efficiency of edge infrastructure, which is especially important given the edge's resource scarcity for power and space reasons~\cite{alibaba_luoshen_nsdi24}.


\Para{Roadmap.} 
As AI pipelines become more and more complex, seamless and efficient offload tools will free AI developers from the burden of worrying about the underlying details of these smart network hardware devices.
Moving forward, our goal is to automate the generation of data processing tasks for SmartNICs.
Can we build a compiler that successfully maps a data processing specification to a semantically equivalent implementation that runs within the 
within resource constraints?
How do we support a diverse set of different data processing operations and hardware backends?

==> evaluation.tex <==


\section{Evaluation}
\label{sec:evaluation}







\begin{figure}
    \centering
    \includegraphics[width=0.95\columnwidth]{figures/final_overhead_results.pdf}
    \vspace{9pt}
    \caption{CPU utilizations after offloading select CPU data processing tasks.}
    \label{fig:cpu-overhead-result}
\end{figure}


\subsection{CPU utilization savings}

To measure the benefits of offloading to SmartNICs, we compare the CPU utilizations of representative vision pipelines with and without offloading \texttt{ToTensor}.
We save the evaluation of offloading other data processing tasks for future work.
We use an SLO of 1 second and scale frame rates based on the compute workloads, which are based on recent industry pipeline studies \cite{gemel}. 
In practice, these frame rates are between 20 -- 30 requests per second which reflects the rates used in prior literature \cite{madeye,chameleon}.
The CPU utilization results are in Figure~\ref{fig:cpu-overhead-result}.
Each experiment was executed for two minutes and the reported CPU utilizations are averages over that time period. 
Overall, we find that offloading is extremely beneficial for significantly reducing the load on inference server CPUs thereby freeing up compute resources for new tasks and requests. 

We observe that as the pipeline gets deeper with more models, the relative savings from offloading the pre-processing operations of the model at the beginning of the DAG is much lower.
We anticipate similar trends to be present for wider, multi-modal models.
For all three of our multi-stage pipelines (car make, person ID, and dog breed), offloading \texttt{ToTensor} from the first model in the DAG improves to a lesser degree.
This is because the total amount of data processing that the pipeline has to perform is considerably higher because each model requires its own data processing operations.
Thus it is necessary to offload pre-processing operations from all models to fully reap CPU utilization performance wins.


\subsection{FPGA resource overheads}
We evaluate the additional FPGA resources consumed by our implementation of tensor conversion compared with the baseline NetFPGA design. We observe that we to meet timing at 200 MHz (clock period of 5 ns). We report the additional FPGA resources consumed by our hardware design in Table~\ref{tab:fpga_resources}. Our resource consumption is modest in comparison to the available resources on the FPGA with many FPGA boards containing an even larger number of resources showing that our design is tenable for many FPGAs available today. Most of the additional resource consumption comes from storage-related resources such as Block RAMs and LUTs are used for the integer to float data type conversion lookup table.

\begin{table}[t]
\footnotesize
\centering
\begin{tabular}{|l|r|r|} 
\hline
\textbf{Resource} & \textbf{\texttt{ToTensor}} & \textbf{Available} \\\hline
\textbf{LUT} & 6191 & 433200 \\\hline 
\textbf{LUTRAM} & 1 & 174200 \\\hline 
\textbf{FF} & 6927 & 866400 \\\hline
\textbf{BRAM} & 27 & 1470 \\\hline
\end{tabular}
\vspace{20pt}
\caption{The utilization of the \texttt{ToTensor} module based on NetFPGA running on an XC7VX690T.}
\label{tab:fpga_resources}
\end{table}

==> offloading.tex <==
\section{How to offload?}


Naively porting data processing operations from the CPU to a network accelerator is not straightforward.  \rn{say more about what this section is talking about before going into the details} \mw{Added an overview in the next few sentences}
In this section, we formalize the process of generating an offloaded SmartNIC implementation as well as the resource constraints of the device that must be satisfied.
We then provide several examples of popular data processing functions used today and why offloading them is not as easy as it may initially seem.


We denote $\textbf{Spec}$ to be a function specification that takes as input a data sample $\vec{x}$ and applies a transformation to it. 
Given an input sequence of $n$ uniformly sized packets $\{\vec{p_n}\}$ and an initial state $\vec{s_0}$ where $\bigcup_{i=0}^n \vec{p_i} = \vec{x}$, our goal is to generate an offloaded implementation $\textbf{Impl}$ that is equivalent to $\textbf{Spec}$ that will be executed on the network accelerator.

\[ \textbf{Spec}(\vec{x}) = \textbf{Impl}(\{\vec{p_n}\}, \vec{s_0} )\]

We denote the function $\textbf{E}$ to capture the resource overheads and program performance incurred by \textbf{Impl}. 
Our goal is to generate a function \textbf{Impl} that minimizes $\textbf{E}$ subject to resource constraints.


\[ \textbf{E}(\textbf{Impl}) := \alpha * \textbf{R}(\textbf{Impl}) + \beta * \textbf{Perf}(\textbf{Impl}) 
\]
\[
\min_{\textbf{Impl}} \textbf{E}(\textbf{Impl}) \quad \text{subject to} 
\]
\[
\quad \textbf{R}(\textbf{Impl}).Memory \leq B
\]


$\textbf{R}$ and $\textbf{Perf}$ represent the resource usage (memory, LUTs, energy) and performance (throughput, latency) of $\textbf{Impl}$. 
$B$ is the upper bound on memory.
For the remainder of this section, we describe several popular data processing functions and attempt to offload them.

\subsection{First Steps in Image Normalization}
The \texttt{Normalize} function is a popular image processing task used for pre-processing images before CNN inference.
It subtracts each pixel value from the mean of its channel and then divides it by the standard deviation of its channel.
We denote $\textbf{I}$ and $\textbf{O}$ as the input and output images respectively and $c$ as the color channel.

\[ \textbf{O}[c,i,j] = \frac{\textbf{I}[c,i,j] - mean[c]} {std[c]} \]

Note that the mean and standard deviation for each channel are normally provided a priori and do not need to be computed.
% Because there are no dependencies within the function, applying the transformation to each packet's data chunk is straightforward, and both data and pipeline parallelism can be achieved.
However, executing these operations incurs significant compute overheads.
\texttt{Normalize} is typically executed after \texttt{ToTensor}, which converts all pixels to 32-bit floating point values.
Performing floating point subtraction and division on each input pixel incurs a substantial amount of clock cycles, which results in considerable energy and resource overheads.
This also causes significant increases in latency and drops in throughput.



\subsection{First Steps in Bilinear Interpolation}
Resizing an image is done via bilinear interpolation.
First, for each output pixel location $(x, y)$, it is necessary to find the four corresponding neigboring pixel locations in the input image using scaling factors $S_x$ and $S_y$.

\[ x_{in} = x * S_x, y_{in} = y * S_y \]
\[ (x_1, y_1) = (\lfloor x_{in} \rfloor, \lfloor y_{in} \rfloor),  (x_2, y_1) = (\lceil x_{in} \rceil, \lfloor y_{in} \rfloor) \] 
\[ (x_1, y_2) = (\lfloor x_{in} \rfloor, \lceil y_{in} \rceil), (x_2, y_2) = (\lceil x_{in} \rceil, \lceil y_{in} \rceil)    \]


In the second step, we compute the output pixel value using the interpolation formula.

\[ 
\begin{split}
\textbf{O}[x,y] = (1 - \Delta_x)(1-\Delta_y)\textbf{I}[x_1, y_1] + \\
\Delta_x(1-\Delta_y)\textbf{I}[x_2, y_1] + \\
(1 - \Delta_x)\Delta_y\textbf{I}[x_1, y_2] + \\
\Delta_x\Delta_y\textbf{I}[x_2, y_2]   
\end{split}
\]

Similar to \texttt{Normalize}, bilinear interpolation incurs significant overheads.
It uses floating point values for its intermediate representations and incurs many multiplication operations for each pixel computation.
Worse, each interpolation operation requires a `tile` of four input pixels which will often not all reside in a single packet.
Because of this, all packets will need to be buffered to reconstruct the image before resizing can occur.
Given a single 1280 x 720 image and an AXI packet size of 256 bits, buffering the entire data sample would require stalling the pipeline to wait for 86400 AXI packets!

\subsection{First Steps in LLM Tokenization}
Text processing begins with text normalization, which performs text transformations such as lowercase conversion and removing special characters.
Tokenization then maps an input text prompt into a series of tokens. 
Below is an example input prompt and its corresponding tokenized sequence.

\vspace{1em}
\noindent
\textbf{Prompt}: This is an example of an input prompt

\noindent
\textbf{Tokens}: ["This", " is", " an", " exam", "ple", " of", " an", " input", " prom", "pt"]
\vspace{1em}


Unlike image normalization, porting tokenization directly onto the network accelerator will not guarantee correctness.
Because the data is split into packets, the device will only see one chunk of the data at a time.
A split could occur at a point that disrupts the continuity of a token yielding an incorrect tokenization result.
Below is an example of chunked tokenization where the word "example" is tokenized differently. 
For simplicity, we use a chunk size 12 bytes and a maximum token length of 5.

\vspace{1em}
\noindent
\textbf{Prompt in chunks}: ["This is an e", "xample of an", "input prompt"] 

\noindent
\textbf{Incorrect tokens}: ["This", " is", " an", " e", "xam", "ple", " of", " an", " input", " prom", "pt"] \\ 
\vspace{1em}

In the correct tokenization, "exam" is a token. 
When the prompt is split, "exam" is divided into different packets and is incorrectly tokenized as "e" and "xam" instead. 
Similar to \texttt{Resize}
Another direct result is that it is difficult to extract parallelism because multiple chunks cannot be tokenized independently. 
Because of these difficulties, naively implementing tokenization results in a lack of correctness and poor performance.



==> scratch.tex <==

- AI is now used to guide or automate decisions in applications across societal sectors, with use cases in healthcare, finance, Internet services, and more. The systems community has played a large role in realizing this revolution. Indeed, the backbone of this success are the model inference platforms that support running ML models, managing user requests and compute resources, as well as managing application data/control flows.

- [the future is distributed...] The most recent wave of AI innovation has brought a heightened need for *distributed* serving of AI pipelines. Reasons include:
** model sizes too large (general LLMs, MoEs): can't fit within single GPUs so aim to parallelize (e.g., tensor parallelism) or disaggregate tasks (prefill and decode) across nodes
** too many iterations (e.g., denoising for image generation, inference-time compute where a single request requires tons of passes through the model): good to distribute to parallelize
** compound AI and agentic pipelines: pipelines are now deeper, with parametric and non-parametric (e.g., vector DBs, verifiers) components that run on different nodes/resources.

- While distribution typically comes with dreaded network delays, this paper argues that it also presents new opportunities to tackle ongoing challenges, namely resource restrictions. [explain insight for why this is useful...]

